Rephrasing natural text data with different languages and quality levels for Large Language Model pre-training

Recently published work on rephrasing natural text data for pre-training LLMs has shown promising results when combining the original dataset with the synthetically rephrased data. We build upon previous work by replicating existing results on C4 and extending them with our optimized rephrasing pipeline to the English, German, Italian, and Spanish Oscar subsets of CulturaX. Our pipeline leads to increased performance on standard evaluation benchmarks in both the mono- and multilingual setup. In addition, we provide a detailed study of our pipeline, investigating the choice of the base dataset and LLM for the rephrasing, as well as the relationship between the model size and the performance after pre-training. By exploring data with different perceived quality levels, we show that gains decrease with higher quality. Furthermore, we find the difference in performance between model families to be bigger than between different model sizes. This highlights the necessity for detailed tests before choosing an LLM to rephrase large amounts of data. Moreover, we investigate the effect of pre-training with synthetic data on supervised fine-tuning. Here, we find increasing but inconclusive results that highly depend on the used benchmark. These results (again) highlight the need for better benchmarking setups. In summary, we show that rephrasing multilingual and low-quality data is a very promising direction to extend LLM pre-training data.

==> figs/fig_rephrasing_diff_models.tex <==
% NOT USED!!!
\begin{figure}[ht]  
\centering 

\begin{tikzpicture}
\begin{axis}[
    %title={CX QA rephrasing at different model scales},
    xlabel={$10^{3}$ steps},
    ylabel={benchmark average},
    xmin=5, xmax=50,
    ymin=48, ymax=58,
    xtick={5,10,15,20,25,30,35,40,45,50},
    xticklabel style = {font=\tiny},%,xshift=0.5ex},
    ytick=      {48,50,52,54,56,58},
    yticklabels={48,50,52,54,56,58},
    yticklabel style = {font=\tiny},%,xshift=0.5ex},
    legend pos=south east,
    legend style={nodes={scale=0.75, transform shape}}, 
    %legend image post style={mark=*},
    ymajorgrids=true,
    grid style=dashed,
    legend style={font=\tiny},
]

% CulturaX EN orig
% https://docs.google.com/spreadsheets/d/1dKQ9g3h44ddC_xTte-011ozY8ztmK21fkXACI6k8x0c/edit?pli=1#gid=872803787 A14
\addplot[
    color=gray,
    line width=1pt,
    ]
    coordinates {
    (5,48.5)(10,51.5)(15,53.4)(20,54.1)(25,55.2)(30,55.3)(35,55.4)(40,55.6)(45,56.2)(50,56.4)
    };

% CX EN 1:1 rephrased QA CORR
% https://docs.google.com/spreadsheets/d/1dKQ9g3h44ddC_xTte-011ozY8ztmK21fkXACI6k8x0c/edit?pli=1#gid=872803787 A182
\addplot[
    color=myRed,
    ]
    coordinates {
    (5,50.2)(10,53.1)(15,55.2)(20,56.2)(25,56.3)(30,56.7)(35,57.0)(40,57.6)(45,57.7)(50,58.0)
    };

% CX EN 1:1 Qwen2 0.5B Instruct rephrased QA CORR
% https://docs.google.com/spreadsheets/d/1dKQ9g3h44ddC_xTte-011ozY8ztmK21fkXACI6k8x0c/edit?pli=1&gid=872803787#gid=872803787 A134
\addplot[
    color=myGreen,
    ]
    coordinates {
    (5,49.1)(10,52.5)(15,54.0)(20,54.9)(25,55.9)(30,55.5)(35,56.4)(40,56.7)(45,56.9)(50,57.1)
    };

% CX EN 1:1 Qwen2 1.5B Instruct rephrased QA CORR
% https://docs.google.com/spreadsheets/d/1dKQ9g3h44ddC_xTte-011ozY8ztmK21fkXACI6k8x0c/edit?pli=1&gid=872803787#gid=872803787 A146
\addplot[
    color=myBlue,
    ]
    coordinates {
    (5,49.9)(10,52.6)(15,54.3)(20,55.5)(25,56.1)(30,56.5)(35,56.5)(40,57.3)(45,56.9)(50,57.4)
    };

% CX EN 1:1 Qwen2 7B Instruct rephrased QA CORR
% https://docs.google.com/spreadsheets/d/1dKQ9g3h44ddC_xTte-011ozY8ztmK21fkXACI6k8x0c/edit?pli=1&gid=872803787#gid=872803787 A158
\addplot[
    color=myPink,
    ]
    coordinates {
    (5,48.5)(10,51.8)(15,53.5)(20,54.6)(25,55.1)(30,55.5)(35,56.0)(40,56.7)(45,56.4)(50,57.0)
    };


\legend{
CX EN (baseline),
CX EN 1:1 re. QA Mistral 7B 0.2v Inst.,
CX EN 1:1 re. QA Qwen2 0.5B Inst.,
CX EN 1:1 re. QA Qwen2 1.5B Inst.,
CX EN 1:1 re. QA Qwen2 7B Inst.,
}

\end{axis}
\end{tikzpicture}% NO EMPTY LINE HERE!!!! 

\caption{Different model scales for QA rephrasing. \michael{Remove at the end, just for info: Only CORRECTED 1:1 runs!}} \label{fig:diffmodels}  
\end{figure}  
